Scaled subordinators and generalizations of the Indian buffet process

We study random families of subsets of $\mathbb{N}$ that are similar to exchangeable random partitions, but do not require constituent sets to be disjoint: Each element of ${\mathbb{N}}$ may be contained in multiple subsets. One class of such objects, known as Indian buffet processes, has become a popular tool in machine learning. Based on an equivalence between Indian buffet and scale-invariant Poisson processes, we identify a random scaling variable whose role is similar to that played in exchangeable partition models by the total mass of a random measure. Analogous to the construction of exchangeable partitions from normalized subordinators, random families of sets can be constructed from randomly scaled subordinators. Coupling to a heavy-tailed scaling variable induces a power law on the number of sets containing the first $n$ elements. Several examples, with properties desirable in applications, are derived explicitly. A relationship to exchangeable partitions is made precise as a correspondence between scaled subordinators and Poisson-Kingman measures, generalizing a result of Arratia, Barbour and Tavare on scale-invariant processes.

==> sec_background.tex <==
\section{Preliminaries}
\label{sec:background}

Suppose we observe data ${X_1,\ldots,X_n}$, say in $\mathbb{R}^d$, and regard each vector $X_i$ as a list of measurements describing an object $i$. A \kword{latent feature model} explains the data using a
${d\times K}$ matrix $\u$ and a ${n\times K}$ binary matrix $\Z$, which parametrize the distribution
of $X$ as
\begin{equation}
  \label{eq:latent:feature:model}
  X_{ij}\sim P_{\phi_{ij}}
  \qquad\text{ where }
  \phi_{ij}:=(\Z_{i1}\u_{jK},\ldots,\Z_{iK}\u_{jK})\;.
\end{equation}
The underlying assumption is that there is unobserved set of $K$ properties, 
called \kword{features}, which each object $i$ may posses (${\Z_{ik}=1}$) or not possess (${\Z_{ik}=0}$). 
Each variable $\Z_{ik}$ acts as a switch that turns the effect of parameter $\u_{jk}$ on $X_{ij}$ on 
or off. If $K$ is fixed and finite, the model is parametric. If $K$ grows unboundedly with the sample size
$n$, so does the total number of parameters affecting the outcomes, and the model is nonparametric. 
In the nonparametric case, the number of features is asymptotically infinite. Since only a finite number of
features, and hence of parameters, should explain any single observation, we generally impose the
constraint 
\begin{equation}
  \label{eq:row:sum:finite}
  \textstyle{\sum_{k}} \Z_{ik}<\infty \qquad\text{for all }i=1,\ldots,n\;.
\end{equation}
A Bayesian latent feature model is defined by specifying a prior distribution on the binary matrix $\Z$
and the parameter matrix $\u$.

The perhaps most widely used example assumes
that the parameters $\u_{ij}$ are scalar effects which combine linearly, and that all additional randomness is additive, independent noise. The model \eqref{eq:latent:feature:model} then takes the form
${X_{ij}\equdist\sum_{k}\Z_{ik}u_{jk} + \varepsilon_{ij}}$,
where $\varepsilon_{ij}$ are independent noise contributions. In statistics, models of this form
are encountered in linear factor analysis. In machine learning and data mining,
they are common in collaborative filtering models, used for example in recommender systems or marketing
applications. See e.g.\ \citep{Griffiths:Ghahramani:2011}
for a review of other applications.

Latent feature models are closely related to clustering models: A clustering solution is a partition
of the input data. A partition of a sample ${X_1,\ldots,X_n}$ can be represented as  partition of its
index set ${\lbrace 1,\ldots,n\rbrace}$. Such a partition can in turn be expressed as a binary matrix $\Z$,
where ${\Z_{ik}=1}$ if $i$ is in cluster $k$, and ${\Z_{ik}=0}$ otherwise. Since each observatioin belongs
to exactly one cluster, this matrix must obey the row sum constraint ${\sum_k\Z_{ik}=1}$ for all $i$,
instead of the finiteness constraint \eqref{eq:row:sum:finite} in the latent feature case.
For example, the two matrices
\begin{center}
\begin{tikzpicture}
  \begin{scope}
    \node at (0,0) {$
      \left(
      \begin{matrix}
        1 & 0 & 0 & 0 & 0 \\
        1 & 0 & 0 & 0 & 0 \\
        0 & 1 & 0 & 0 & 0 \\
        1 & 0 & 0 & 0 & 0 \\
        0 & 0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 1 & 0 
      \end{matrix}\right)
      $};
    \node at (0,1.8) {block \#};
    \node[rotate=90] at (-1.7,0) {object \#};
    \node at (0,-1.8) {partition};
  \end{scope}
  \begin{scope}[xshift=5.5cm]
    %\node at (0,2.9) {\sc Family of sets};
    \node at (0,0) {$
      \left(
      \begin{matrix}
        1 & 0 & 0 & 0 & 0 \\
        1 & 0 & 0 & 0 & 0 \\
        1 & 1 & 0 & 1 & 0 \\
        1 & 0 & 1 & 0 & 0 \\
        0 & 0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 1 & 0
      \end{matrix}\right)
      $};
    \node at (0,1.8) {block \#};
    \node[rotate=90] at (-1.7,0) {object \#};
    \node at (0,-1.8) {family of sets};
  \end{scope}
\end{tikzpicture}
\end{center}
respectively represent the partition and family of sets
\begin{equation}
  (\lbrace 1,2,4 \rbrace,
  \lbrace 3 \rbrace,
  \lbrace 5, 6 \rbrace
  )\;
  \qquad\text{ and }\qquad
  ( 
  \lbrace 1,2,3,4 \rbrace,
  \lbrace 3 \rbrace,
  \lbrace 4,5\rbrace,
  \lbrace 3,6 \rbrace
  )\;.
\end{equation}




\subsubsection*{The Indian buffet process}

The Indian buffet process (IBP) of \citet{Griffiths:Ghahramani:2006}
is a prior distribution
for Bayesian feature models that generates a random family of sets, represented by
a binary ${n\times\infty}$ matrix $\Z$.
Griffiths and Ghahramani originally derived the model as a modification of the Chinese restaurant
process.

For our purposes, a different, equivalent definition is more suitable:
Let $(J_k)$ be an infinite sequence
of random variables with values in $[0,1]$. Given $(J_k)$, a matrix $\Z$ can be generated column-wise as
\begin{equation}
  \label{eq:Bernoulli:sampling:basic}
  \Z_{1k},\ldots,\Z_{nk}|(J_k)\simiid\Bernoulli(J_k) \;.
\end{equation}
The entries of $\Z$ are conditionally independent given $(J_k)$. 
The number of entries in the $i$th row of $\Z$ is the number of variables invoked to explain
the $i$th observation. Since the model is nonparametric, this number should be unbounded, but
remain finite for any given $i$. We hence impose the row-sum condition ${\sum_k\Z_{ik}<\infty}$
a.s.\ for all $i$, which in turn requires ${\sum_k J_k<\infty}$ a.s. 
This implies the variables $J_k$ cannot be i.i.d. They may be independent,
though, and the easiest way to obtain a suitable
sequence is to assume the variable ${\sum_k J_k}$ is infinitely divisible.
The L\'evy-Khinchine theorem then implies
that $J_k$ are the jumps of a subordinator, \ie of an increasing,
pure-jump \Levy process with values in $\mathbb{R}_+$. 
A subordinator is defined by a \Levy density $\rho$. 
%% Equivalently,
%% $J_k$ are the inter-arrival times of a Poisson process
%% with mean measure ${m_{\rho}(ds)=\rho(s)ds}$ on $\mathbb{R}_+$.
If one chooses specifically
\begin{equation}
  \label{eq:density:scale-invariant:interval}
  \rho(s)ds=\theta s^{-1}ds \qquad\text{ for } s\in[0,1] \text{ and some }
  \theta>0\;,
\end{equation}
the resulting matrix $\Z$ has the distribution $\IBP(\theta)$ 
introduced in \citep{Griffiths:Ghahramani:2006}. 

\subsection{Feature models and random measures}

In a Bayesian model, the matrix $\Z$ is used in conjunction with the parameters $U_k$,
and it is hence useful to maintain a joint representation of $(\Z,(U_k))$, since
these variables couple in the posterior. \citet{Thibeaux:Jordan:2007} provided an
elegant solution using random measures: 
Consider a discrete measure ${m=\sum_k j_k\delta_{u_k}}$ on $\atomspace$. Call such
a measure \kword{unitary} if ${j_k\in[0,1]}$ and ${\sum_kj_k<\infty}$.
Given $m$, define a random measure $\Pi$ as
\begin{equation}
  \label{eq:def:BeP}
  \Pi(\argdot):=\sum_{k\in\mathbb{N}} Z_{k}\delta_{u_k}(\argdot)
  \qquad\text{ with } 
  Z_{k}\sim\Bernoulli(w_k) \text{ independently.}
\end{equation}
\citet{Thibeaux:Jordan:2007} call $\Pi$ a \kword{Bernoulli process} with parameter
${m}$, denoted $\BeP(m)$ in the following. To generate the pair ${(\Z,(U_k))}$, we
randomize $m$ by defining a random unitary measure 
\begin{equation}
  \mu:=\sum_{k} J_k\delta_{U_k}\;,
\end{equation}
and sample 
\begin{equation}
  \label{eq:BeP:sampling}
  \Pi_1,\ldots,\Pi_n|\mu\simiid\BeP(\mu)\;.
\end{equation}
Each random measure $\Pi_i$ is of the form ${\Pi_i=\sum_{k}\Z_{ik}\delta_{U_k}}$, and corresponds to the
$i$th row of $\Z$. All $\Pi_i$ share the same sequence $(U_k)$ of atom locations.

%% Once again, one usually tries to avoid dependencies between the constituent variables of $\mu$,
%% because such dependencies would constitute an additional modeling assumption, and because
%% even simple dependencies in the prior can result in complex dependencies in the posterior.
%% Of particular interest are hence random measures in which the variables $U_k$ are \iid
%% and independent of the sequence $(J_k)$. Such random measures are called \kword{homogeneous}.

A random measure ${\mu=\sum J_k\delta_{U_k}}$ is called \kword{homogeneous} if 
the variables $U_k$ are \iid and independent of the sequence $(J_k)$.
If the weights $(J_k)$ of a homogeneous random measure $\mu$ are the jumps of a subordinator,
$\mu$ is a (homogeneous) \kword{completely random measure} (CRM) in the sense of \citet{Kingman:1967}. 
Although this does not technically exhaust the class of CRMs, it is sufficient for all
problems considered in the following, and all CRMs used in the following are assumed
to be homogeneous. A homogeneous CRM is determined by the law $G$ of $U_1$
and by the \Levy density $\rho$ of the defining subordinator. Since the relevant properties
are completely specified by $\rho$, it is customary to neglect $G$.

If $\mu$ is chosen as a \kword{beta process}, a CRM introduced by \citet{Hjort:1990},
one obtains a two-parameter generalization of the IBP first proposed by 
\citet{Ghahramani:Griffiths:Sollich:2006:1}.
\citet{Teh:Goerur:2009} introduced a third parameter
which controls the distribution of the column sums of $\Z$ (\ie of the number of
observations exhibiting each feature); suitable parameter settings result in a
power law distribution. This model, called a \kword{stable-beta process}
in \citep{Teh:Goerur:2009}, has \Levy density
\begin{equation}
  \label{eq:beta:stable:process}
  \rho(s)ds=\frac{c}{B(\alpha+\gamma,1-\alpha)}
  s^{-\alpha-1}(1-s)^{\gamma+\alpha-1}ds
  \qquad\text{ for }c,\theta>0 \text{ and }\alpha>-\gamma\;,
\end{equation}
where $B$ is the beta function; this \Levy density first appeared 
in \citep{Kim:Lee:2003}.
Choosing ${\alpha=0}$ yields the two-parameter beta process. Additionally choosing
${\gamma=1}$ yields \eqref{eq:density:scale-invariant:interval},
and hence the original, one-parameter IBP.




